Whence to Learn? Transferring Knowledge in Configurable Systems using BEETLE

As software systems grow in complexity and the space of possible configurations increases exponentially, finding the near-optimal configuration of a software system becomes challenging. Recent approaches address this challenge by learning performance models based on a sample set of configurations. However, collecting enough sample configurations can be very expensive since each such sample requires configuring, compiling, and executing the entire system using a complex test suite. When learning on new data is too expensive, it is possible to use \textit{Transfer Learning} to "transfer" old lessons to the new context. Traditional transfer learning has a number of challenges, specifically, (a) learning from excessive data takes excessive time, and (b) the performance of the models built via transfer can deteriorate as a result of learning from a poor source. To resolve these problems, we propose a novel transfer learning framework called BEETLE, which is a "bellwether"-based transfer learner that focuses on identifying and learning from the most relevant source from amongst the old data. This paper evaluates BEETLE with 57 different software configuration problems based on five software systems (a video encoder, an SAT solver, a SQL database, a high-performance C-compiler, and a streaming data analytics tool). In each of these cases, BEETLE found configurations that are as good as or better than those found by other state-of-the-art transfer learners while requiring only a fraction ($\frac{1}{7}$th) of the measurements needed by those other methods. Based on these results, we say that BEETLE is a new high-water mark in optimally configuring software.

==> RQ4.tex <==
\begin{figure}[htbp!]
{\small
    \begin{minipage}[]{\linewidth}
    \textbf{{\sc Sac}}\\[0.01cm]
    \resizebox{\linewidth}{!}{% 
    \begin{tabular}{|llrrc|}
    \arrayrulecolor{lightgray}
    \rowcolor{lightgray}{\small \textbf{Rank}} & {\small\textbf{Learner}} & {\small \textbf{Median}} & {\small\textbf{IQR}} & \\\hline  
    \rowcolor{lightergray}  1 &       Jamshidi \etal~\cite{jamshidi2017transfer} &    1.58  &  5.39 & \quart{0}{4}{0}{0} \\\hline
      2 &     Baseline &    6.89  &  99.1 & \quart{0}{79}{5}{0} \\
      2 &     Valov \etal~\cite{valov2017transferring} &    6.99  &  99.24 & \quart{0}{79}{6}{0} \\
    \hline \end{tabular}}\\[0.01cm]
    \textbf{{\sc Spear}}\\[0.01cm]
    \resizebox{\linewidth}{!}{%
    \begin{tabular}{|llrrc|}
    \arrayrulecolor{lightgray}
    \rowcolor{lightgray}{\small \textbf{Rank}} & {\small\textbf{Learner}} & {\small \textbf{Median}} & {\small\textbf{IQR}} & \\\hline  
    \rowcolor{lightergray}  1 &       Jamshidi \etal~\cite{jamshidi2017transfer} &    0.70  &  1.29 & \quart{0}{0}{3}{0}\\
    \rowcolor{lightergray}1 &     BEETLE &    0.79  &  1.40 & \quart{0}{0}{3}{0} \\
    \rowcolor{lightergray}1 &     Valov \etal~\cite{valov2017transferring} &    1.11  &  1.98 & \quart{0}{2}{4}{0} \\
    \hline\end{tabular}}\\[0.01cm]
    \textbf{{\sc SQLite}}\\[0.05cm]
    \resizebox{\linewidth}{!}{%%
    \begin{tabular}{|llrrc|}
    \arrayrulecolor{lightgray}
    \rowcolor{lightgray}{\small \textbf{Rank}} & {\small\textbf{Learner}} & {\small \textbf{Median}} & {\small\textbf{IQR}} & \\\hline  
    \rowcolor{lightergray}  1 &     BEETLE &    5.41  &  9.28 & \quart{2}{10}{5}{0} \\\hline
      2 &     Valov \etal~\cite{valov2017transferring} &    6.96  &  12.91 & \quart{3}{15}{6}{0} \\
      3 &     Jamshidi \etal~\cite{jamshidi2017transfer}   &    18.51  &  50.85 & \quart{2}{50}{18}{0} \\
    \hline \end{tabular}}\\[0.01cm]
    \textbf{{\sc Storm}}\\[0.01cm]
    \resizebox{\linewidth}{!}{%
    \begin{tabular}{|llrrc|}
    
    \arrayrulecolor{lightgray}
    \rowcolor{lightgray}{\small \textbf{Rank}} & {\small\textbf{Learner}} & {\small \textbf{Median}} & {\small\textbf{IQR}} & \\\hline  
    \rowcolor{lightergray}    1 &     BEETLE &    0.04  &  0.06 & \quart{0}{0}{0}{0} \\\hline
      1 &       Jamshidi \etal~\cite{jamshidi2017transfer} &    0.86  &  20.69 & \quart{0}{21}{1}{0} \\
      2 &     Valov \etal~\cite{valov2017transferring} &    2.47  &  53.98 & \quart{0}{54}{4}{0} \\
    \hline \end{tabular}}\\[0.01cm]
    \textbf{{\sc x264}}\\[0.01cm]
    \resizebox{\linewidth}{!}{%
    \begin{tabular}{|llrrc|}
    \arrayrulecolor{lightgray}
    \rowcolor{lightgray}{\small \textbf{Rank}} & {\small\textbf{Learner}} & {\small \textbf{Median}} & {\small\textbf{IQR}} & \\\hline  
    \rowcolor{lightergray}  1 &     BEETLE &    8.67  &  27.01 & \quart{2}{31}{8}{0} \\\hline
      2 &     Valov \etal~\cite{valov2017transferring} &    16.99  &  41.24 & \quart{5}{47}{17}{0} \\
      3 &       Jamshidi \etal~\cite{jamshidi2017transfer} &    43.58  &  28.39 & \quart{34}{48}{44}{0} \\
    \hline \end{tabular}}
    \end{minipage}}
    \caption{{\small Comparison between state-of-the-art transfer learners and BEETLE. The best transfer learner is shaded \colorbox{lightergray}{gray}.}}
    \label{fig:rq4}
    \end{figure}
    
    \begin{figure}[t]
        \centering
        \includegraphics[width=0.95\linewidth]{figures/Measurements.png}
        \caption{{\small BEETLE v/s  state-of-the-art transfer learners. The numbers in parenthesis represent the numbers of measurements BEETLE uses in comparison to the  state-of-the-art learners.}}
        \label{fig:rq4_measurement}

\end{figure}

==> approach1.tex <==
\begin{figure*}[htbp]
\centering
\begin{subfigure}[t]{0.45\linewidth}
\centering
\textbf{Pick Bellwether Environment}\\[0.5cm]
\includegraphics[width=\linewidth]{figures/source_target.png}
\end{subfigure}\hspace{5pt}
\begin{subfigure}[t]{0.5\linewidth}
\hspace{0.4\linewidth}\textbf{Pseudocode}
\small
\begin{lstlisting}[xleftmargin=8.0ex,mathescape,frame=none,numbers=left]
def FindBellwether(sources, step_size, budget, thres, lives): 
  while lives or cost > budget:
    "Sample configurations"
    sampled = list()
    for source in sources:
      sampled += source.sample(step_size)
    "Get cost"
    cost = get_cost(sampled)
    "Evaluate pair-wise performances"
    perf = get_perf(sampled)
    "Remove non-bellwether environments"
    sources = remove_non_bellwethers(sources, perf, thres)
    "Loose life if no sources are removed"
    if prev == len(sources): lives -= 1
    "Return a bellwether"
  return sources[argmin(perf)]
\end{lstlisting}
\end{subfigure}\\[0.4cm]
\begin{subfigure}[t]{0.5\linewidth}
\centering
\textbf{Transfer Learning with Bellwether Environment}\\
\includegraphics[width=0.85\linewidth]{figures/bellwether-transfer.png}
\end{subfigure}~~%
\begin{subfigure}[t]{0.5\linewidth}
\vspace{0.4cm}
\hspace{0.4\linewidth}\textbf{Pseudocode}\\[-0.3cm]
\small
\begin{lstlisting}[xleftmargin=5.0ex,mathescape,frame=none,numbers=left]
def BEETLE(sources, target, budget): 
    "Find the bellwether environment"
    bellwether = FindBellwether(sources, step_size, budget, thres, lives)
    "Sample the bellwether source to fit budget"
    b_some = bellwether.sample(budget)
    "Train a prediction model with the bellwether"
    prediction_model = regTree.train(b_some)
    predicted = prediction_model.test(target.indep)
    return target[argmin(predicted)]
\end{lstlisting}
\end{subfigure}	
\caption{{\small This figure demonstrates the two key aspects of our proposed approach for transfer learning (a)~how to pick the bellwether environment; (b)~How to construct a  transfer learner with the bellwether environment. A visual intuition of each of the two methods is presented on the left and the corresponding pseudocode are presented on the right.}}
\label{fig:approach}
\end{figure*}

==> body/response.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%                               RESPONSE TO REVIEWERS
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\pagebreak
\newpage
\pagenumbering{gobble}
\renewcommand*{\thesection}{\Alph{section}}
\balance
\section*{RESPONSE TO REVIEWERS}
\section*{Comments from the editor}

\review{There are still a few minor revision requests from the reviewers regarding the time complexity / discussion about near optimal and real optimal / discussion on comparisons / highlight the aspects of methods and configuration of uses. Therefore, I recommend a minor revision. Please address the comments by R1 and R3.}

Thank you very much. We have made appropriate changes to the manuscript as requested by the reviewers. Below are the summary of the changes:
\bi
  \item \bareresp{2-1}: Here we have present the discussion on the computational complexity of the algorithm.
  \item \bareresp{3-1}: Here we highlight the methodological question from review 3 regarding the implication of fig 3b.
\ei
\hfill
\section*{Reviewer 2}

\review{(2-1) I posed this question in my previous review, and you show that the tool is easy to use. Since you mention “the effect of BEETLE on the day to day business of a software engineer”, what is the time complexity of this tool?}

Thanks for highlighting this. In order to understand the computational complexity, we compare our method with those of previous approaches \cite{krishna16, krishna18}. We note that \tool offers noticible speedups. Specifically, given that we have $\mathit{M}$ enviroments and $\mathit{n}$ measurements in each enviroment, we may categorize the speedups offered by \tool into the following cases:
\bi
\item {\em Best Case:} Here, we expect the racing algorithm of \tool to eliminate atleast half of the non-bellwether enviroments at every iteration. This gives us a recurrence relation of $T(M) = T(M/2) + f(n)$, which gives us a best case complexity of $\mathit{O(log_2(M)\cdot f(n))}$. 
\item {\em Worst Case:} Here, we expect the racing algorithm of \tool to eliminate \textit{just one} non-bellwether enviroment at every iteration. This gives us a recurrence relation of $T(M) = T(M-1) + f(n)$, which gives us a worst case complexity of $\mathit{O(M^2 \cdot f(n))}$. Note that this worst case is same as the complexity of \cite{krishna16, krishna18}.  
\ei

In practice, we note that the average case speedup is somewhere in between that of the best case (i.e., $\mathit{O(log_2(M)\cdot f(n))}$) and the worst case (i.e., $\mathit{O(M^2 \cdot f(n))}$).
We have added this text in our draft~\citeresp{2-1}.\\

\review{(2-2) In RQ3, the authors show the BEETLE outperforms the non-transfer learning algorithm based on their win/loss ratios. But they didn’t conduct similar comparisons between BEETLE and the state-of-art techniques. I would like to see some discussions about this.}

We apologize for the confusion here. We chose to compute the win-loss ratio for \tool vs. non-transfer based approach of Nair \etal~\cite{nair2017faster} inorder to compare the success rate of \tool vs. Nair \etal's method at various sampling percentages ranging from 10\% to 100\%. Having established that \tool outperforms Nair \etal's method in RQ3 and that that we only need $\approx13.5\%$ of the samples to discover the bellwether enviroment(s) in RQ2, we chose to use present the Scott-Knott ranking of \tool as compared to other state of the art methods in Fig. 9. We also present the comparison of the number of samples used in Fig. 10.     \\

\review{(2-3)~This is just a minor issue. The paper presents a tool to find the near-optimal configurations, but I didn’t find any discussion about the difference between near-optimal and real-optimal configurations. I am fine with the methodology in this paper, but I am still curious that how closed of the configurations found by BEETLE to the real-optima.}

This is a great question. Unfortunately, true global optima is very hard to determine without having to exhaustively search the configuration space. As an example, in $\mathit{SaC}$ there are 50 configurable parameters. Even if we assume that all the parameters are boolean (which is not true in reality), we still have $2^50$ possible configurations. This is very large number of configurations to be able to exhaustively search to determine the global optima.  \\

\section*{Reviewer 3}

We would like to thank you very much for your detailed review and your comments. We have addressed the remainder of you concerns in this draft. 

\review{(3-1) If I correctly understand, in the following scenario: I have a *new*"environment" (target) for my configurable system, what should I do? The answer is that you don't compare the best predicted performance with configuration measurements in the target. You "trust" the bellwether(s) can generalize and pick one.  I strongly recommend to better highlight this aspect of the method (in Section 4) and to avoid confusions. For example, Figure 3b has several "target environments", giving the overall impression that you need to measure some configurations even in the targets.}

That is correct-- If we have a *new* ``environment'' (target) for a configurable system, then we don't make any configuration measurements in the target, instead, we just "trust" the bellwether(s) can generalize and pick one.

We have updated our paper with this change in \S4~\citeresp{3-1}.\hfill\\

\review{(3-2) ``A fraction (about 1\%) of all available data is sampled. A
prediction model is built with these sampled datasets.'' Where does this 1\% comes from? It seems not aligned with the 10\% of the empirical results}

\noindent We do apologize, this was a typo. We have fixed this. 

\hfill

\section*{Reviewer 1}

We thank you very much for your review and your comments!

==> cost_x264.tex <==
\begin{figure}[t!]
    \centering
    \includegraphics[width=.8\linewidth]{cost_x264.png}
    \caption{\small }
    \label{fig:cost_x264}
\end{figure}

==> pooyan_pseudo.tex <==
\begin{figure}[t]
\small
\begin{lstlisting}[xrightmargin=6ex, mathescape,frame=none,numbers=right]
def GPTransform(source, target, source_budget, target_budget): 
  "Sample random configurations"
  s_some = source.sample(source_budget)
  t_some = target.sample(target_budget)
  "Get performance measurements"
  s_perf = get_perf(s_some)
  t_perf=get_perf(t_some)
  "Compute correlation"
  perf_correlation = get_correlation(s_perf, t_perf)
  "Compute covariance"
  input_covariance = get_covariance(s_some, t_some)
  "Construct a kernel"
  kernel = input_covariance $\times$ perf_correlation
  "Train the Gaussian Process model"
  learner = GaussianProcessRegressor(kernel)
  prediction_model = learner.train(s_some)
  return prediction_model
\end{lstlisting}
\caption{\small{Gaussian Process Transformation Transfer. From   Jamshidi \etal~\cite{jamshidi2017transfer}.}}
\label{fig:gptransform}  
\end{figure}


==> trees.tex <==

 
 Another specific aspect of our design is how we measure model {\em comprehensible}. 
We assume that software engineers will want to browse and understand and audit the results of any
 algorithm that has the presumption to tell them to change this our that.
 One way to present the results of an optimizer is to generate a {\em domination tree}, as fp;;pws"
 \bi
 \item
 Take all the examples
 ever evaluated by the optimizer; 
 \item
 Score each individual  by $|\Omega_I(x)|$, which is the number
 of other individuals dominated by $x$; 
 \item
 Use the CART decision tree learner~\cite{breiman1984classification} to summarize the
 decisions that lead to difference domiantion scores.
 \ei
  In
 this paper, we will say domination trees with {\em fewest} nodes and leaves
 are {\em more} comprehensible. 
 For example, Figures~\ref{fig:dom1} and~\ref{fig:dom2} show two trees generated from
 the examples evaluated by FLASH and ePAL while optimizing the SS1 model of 
 Figure~\ref{fig:unconstrained_case_studies}.
 Note that one of these trees is far smaller  and hence easier
 to browse, understand, and audit.
 
  
 
 \begin{figure}[!b]
 \renewcommand{\baselinestretch{0.65}}
\hspace{0.2cm}\begin{lstlisting}[
escapechar=@,
basicstyle=\scriptsize\ttfamily,
keepspaces=true,
linewidth=3.25in,
frame=none,
numbers=right]
@\bh@sccp=0@\eh@
|    print_used_types=0
|    |    ipsccp=0 (6.5)
|    |    ipsccp=1
|    |    |    x[10]=0 (12) 
|    |    |    x[10]=1 (19) 
|    @\bh@print_used_types=1@\eh@
|    |    ipsccp=0 (14)
|    |    @\bh@ipsccp=1@\eh@
|    |    |    time_passes=0  (24)
|    |    |    @\bh@time_passes=1@\eh@
|    |    |    |    jump_threading=0 (28)
|    |    |    |    @\bh@jump_threading=1@\eh@ (31)
sccp=1
|    ipsccp=0 (1.5) 
|    ipsccp=1 (7.5) 
\end{lstlisting}
\caption{\small{A domination 
tree. Optimizer = FLASH; model= SS1, from Figure~\ref{fig:unconstrained_case_studies}.
Numbers in brackets (e.g. ``(31)'') show how many other individuals are dominated by individuals in a particular leaf.
For example, on the last line, there is a leaf whose individuals dominate (on average)
31 others.
The branch marked in gray leads to the branch with greatest score.
}}\label{fig:dom1}  
\end{figure}
 
 \begin{figure}[!b]
\renewcommand{\baselinestretch{0.65}}
\hspace{0.2cm}\begin{lstlisting}[
escapechar=@,
basicstyle=\scriptsize\ttfamily,
keepspaces=true,
linewidth=3.25in,
frame=none,
numbers=right]
ipsccp=0
|    iv_users=0
|    |    sccp=0
|    |    |    print_used_types=0
|    |    |    |    jump_threading=0
|    |    |    |    |    time_passes=0
|    |    |    |    |    |    instcombine=0 (16)
|    |    |    |    |    |    instcombine=1 (12)
|    |    |    |    |    time_passes=1
|    |    |    |    |    |    instcombine=0 (10)
|    |    |    |    |    |    instcombine=1 (11)
|    |    |    |    jump_threading=1
|    |    |    |    |    gvn=0
|    |    |    |    |    |    inline=0
|    |    |    |    |    |    |    simplifycfg=0 (22)
|    |    |    |    |    |    |    simplifycfg=1 (20)
|    |    |    |    |    |    inline=1 (26)
|    |    |    |    |    simplifycfg=0 (32)
|    |    |    |    |    simplifycfg=1 (33)
|    |    |    print_used_types=1
|    |    |    |    |inline=0 (47)
|    |    |    |    |inline=1 (43)
|    |    sccp=1
|    |    |    print_used_types=0 (1)
|    |    |    |print_used_types=1 (7)
|    iv_users=1
|    |    sccp=0
|    |    |    print_used_types=0
|    |    |    |    jump_threading=0 (30)
|    |    |    |    jump_threading=1 (42)
|    |    |    print_used_types=1
|    |    |    |    inline=0 (56)
|    |    |    |    inline=1 (62)
|    |    sccp=1
|    |    |    instcombine=0 (26)
|    |    |    instcombine=1 (33)
@\bh@ipsccp=1@\eh@
|    @\bh@sccp=0@\eh@
|    |    print_used_types=0
|    |    |    iv_users=0
|    |    |    |    jump_threading=0 (50)
|    |    |    |    jump_threading=1 
|    |    |    |    |    instcombine=0 (53)
|    |    |    |    |    instcombine=1 (54)
|    |    |    iv_users=1
|    |    |    |    simplifycfg=0 (59.5)
|    |    |    |    simplifycfg=1 
|    |    |    |    |    time_passes=0 (63)
|    |    |    |    |    time_passes=1 (66)
|    |    @\bh@print_used_types=1@\eh@
|    |    |    iv_users=0
|    |    |    |    time_passes=0 (69)
|    |    |    |    time_passes=1
|    |    |    |    |    instcombine=0 (73)
|    |    |    |    |    instcombine=1 (71)
|    |    |    @\bh@iv_users=1@\eh@
|    |    |    |    gvn=0 (76)
|    |    |    |     @\bh@gvn=1 (79)@\eh@
|    sccp=1
|    |    print_used_types=0
|    |    |    jump_threading=0 (3)
|    |    |    jump_threading=1 (16)
|    |    print_used_types=1
|    |    |    iv_users=0 (35)
|    |    |    iv_users=1 (50)
\end{lstlisting}
\caption{\small{Another domination tree. Same
format as Figure~\ref{fig:dom1} but the optimizer is ePAL.
This tree is larger than Figure~\ref{fig:dom1}
(and hence harder to understand) since ePAL evaluated more examples than FLASH.
}}\label{fig:dome2}  
\end{figure}
 
 
 

==> waterloo_peudo.tex <==
\begin{figure}[t]
\small
\begin{lstlisting}[xrightmargin=6ex, mathescape,frame=none,numbers=right]
def LinearTransform(source, target, 
                    training_coef, budget): 
  "Construct a prediction model"
  prediction_model=regTree.train(source, training_coef)
  "Sample random measurements"
  s_samp = source.sample(budget)
  t_samp = target.sample(budget)
  "Get performance measurements"
  s_perf=get_perf(s_samp)
  t_perf=get_perf(t_samp)
  "Train a transfer model with LR"
  transfer_model=linear_model.train(s_perf, t_perf)
  return prediction_model, transfer_model
\end{lstlisting}
\caption{\small{Linear Transformation Transfer. From Valov \etal~\cite{valov2017transferring}.}}
\label{fig:lineartransform}  
\end{figure}
